Strong Anonymity for Mesh Messaging

Messaging systems built on mesh networks consisting of smartphones communicating over Bluetooth have been used by protesters around the world after governments have disrupted Internet connectivity. Unfortunately, existing systems have been shown to be insecure; most concerningly by not adequately hiding metadata. This is further complicated by the fact that wireless communication such as Bluetooth is inherently a broadcasting medium. In this paper, we present a new threat model that captures the security requirements of protesters in this setting. We then provide a solution that satisfies the required security properties, hides all relevant metadata, scales to moderately sized protests, and supports group messaging. This is achieved by broadcasting all messages in a way that limits the overhead of duplicate messages, ensuring that ciphertexts do not leak metadata, and limiting what can be learned by observing user behavior. We also build a model of our system and numerically evaluate it to support our claims and analyze how many users it supports. Finally, we discuss further extensions that remove potential bottlenecks in scaling and support substantially more users.

==> ideal_functionality.tex <==
\noindent\fbox{\begin{minipage}{\dimexpr0.45\textwidth-2\fboxsep-2\fboxrule\relax}

\emph{Ideal Functionality} \\

\neil{I don't think we need to allow A to add nodes. It seems the same as A having them there at the beginning but having no edges to them and just adding the edges later.} \\
Let $G$ be a graph that an adversary $A$ controls. $A$ can add edges, remove edges, and add nodes to $G$. \\

Let $F$ be an ideal functionality that works as follows: \\

First, $F$ has a registration phase where parties give $F$ their public keys and $turn$ values. $A$ sends $F$ a list of which parties it controls. $F$ then sends $A$ a list of all $turn$ values with mappings to nodes in $G$. \\

Then, over a series of $t$ rounds, parties interact with $F$ by sending it ($message$, $recipient$) where $message$ is some message and $recipient$ is a public key. \\

At the beginning of round $i$, where $i \in [1,...,t]$, $F$ reads the current state of $G$ and stores it as $G_i$. \\

When $F$ receives ($message$, $recipient$) from a party $p$ on round $i$, $F$ checks if $recipient$ is controlled by $A$ and if it is, it delivers $message$ to $A$. If $recipient$ is not controlled by $A$, then $F$ chooses a random number $x$ from [1, max\_delay], where max\_delay is some constant representing the maximum number of rounds that a message can be delayed, and gives $message$ to $recipient$ on round $i + x$ only if there is a \emph{good path} from $p$ to $recipient$ in $G_i, ..., G_{i + x}$.

\end{minipage}
}

\noindent\fbox{\begin{minipage}{\dimexpr0.45\textwidth-2\fboxsep-2\fboxrule\relax}
\emph{Good Path} Definition: \\

The set of graphs $G_1, ..., G_n$ has a \emph{good path} from $a$ to $b$ if a path can be walked from $a$ to $b$ by only using edges in $G_i$ for the $i$th edge in the path. We allow the walk to ``pause'' or ``wait'' by taking no edge (equivalent to taking a self edge) in the $i$th round.\\

Note that direction matters, i.e. there may be a \emph{good path} from $a$ to $b$ but not from $b$ to $a$ in a sequence of graphs.https://www.overleaf.com/project/60a2f12a0ac95616d1467d09
\end{minipage}
}

==> simulation_proof.tex <==
% %A lives in the ideal world and wants to simulate the real world.

% \noindent We construct an efficient simulator $S$ that works as follows:

% \noindent$A$ gives $S$ a list of public parameters that include $send\_rate$, $DS_{share}$, $time\_to\_keep$, and the number of time epochs $t$ to simulate. $A$ also gives $S$ a list of corrupted devices $M$ with arbitrarily chosen $turn$ values, $DS$s, and public/secret key pairs for each device.

% \noindent$S$ will have honest nodes discard any data they receive that they do not know how to interpret.

% \noindent$S$ initializes the message history transcript $transcript$ to a list containing $t$ empty sets.

% \noindent$S$ initializes an empty list of honest devices called $H$.

% \noindent$S$ does the following for each time epoch $i$ in $[1, ..., t]$:

% % how to handle A adding honest vs malicious nodes?
% % A sends new graph
% \noindent$S$ waits for $A$ to provide $G_i$. $S$ adds any new honest nodes to $H$ and any new malicious nodes to $M$.
% For each new honest node, $S$ chooses a uniformly random value from $[1, send\_rate)$ for its $turn$ value and initializes its $DS$ to a new empty one.

% \noindent$S$ waits for $A$ to provide an order to execute the following steps (they can be interleaved, i.e. some of 1, then some of 2, then some of 1, then some of 6, etc.):

% \begin{adjustwidth}{1cm}{}
% % generate messages
% % instantaneous sending?
% % instead of adding things to malicious neighbors, just notify A
% \noindent (1) For each node $p$ in $H$, $S$ checks if $i$ \ms{\%} $send\_rate$ == $p.turn$ and if it is $True$, adds $(E(PK_{dummy}, 0), i)$ to $p.DS$ and $p$'s honest neighbors' DSs. $S$ informs $A$ which malicious nodes received data and what they received. $S$ then inserts $((E(PK_{dummy}, 0), i), p, p.neighbor)$ into $transcript[i]$ for each neighbor.

% % share DS
% \noindent (2) For each node $p$ in $H$, $S$ checks if $i - p.turn$ $\%$ $DS_{share} == 0$ and if it is $True$ adds all of the message digests to $p$'s honest neighbors' missing messages list. $S$ informs $A$ which malicious nodes received data and what they received. $S$ then inserts $(p.DS, p, p.neighbor)$ into $transcript[i]$ for each neighbor.

% % ask for missing messages
% \noindent (3) For each node $p$ in $H$, $S$ checks if $p$ has any missing messages and sends message requests to each of $p$'s honest neighbors. $S$ informs $A$ which malicious nodes received data and what they received. $S$ then inserts $(Requests, p, p.neighbor)$ into $transcript[i]$ for each neighbor.

% % respond to missing messages
% \noindent (4) For each node $p$ in $H$, $S$ checks if $p$ has any message requests and if it does, sends each message from the request to each of $p$'s honest neighbors who add it to their $DS$. $S$ informs $A$ which malicious nodes received data and what they received. $S$ then inserts $((Message), i), p, p.neighbor)$ into $transcript[i]$ for each message and neighbor.

% % clean up $DS$
% \noindent (5) For each node $p$ in $H$, $S$ removes all messages older than $time\_to\_keep$ from $p.DS$. \\

% \noindent (6) For each node $m$ in $M$, $S$ queries $A$ for $m$'s behavior. $m$ can send arbitrary data to its neighbors (messages or digests) as well as add, remove, or modify data from its storage. $S$ then inserts $(data, m, m.neighbor)$ into $transcript[i]$ for each neighbor.

% \end{adjustwidth}

% In the execution of the real protocol, real messages and cover traffic (0 encrypted with a dummy key) are indistinguishable due to the properties of the underlying cipher and follows from a hybrid argument. Therefore, all messages in the execution of the real protocol can be viewed as cover traffic. In the simulation, only cover traffic is sent. The distribution of cover traffic in the execution of the real protocol is identical to the distribution of cover traffic sent in the simulation. The distribution of $turn$ values is also equivalent (honest users choose them from a uniform random distribution and malicious users choose them arbitrarily). Since the distribution of other traffic such as the exchange of digests and reliable message delivery depends solely on the distribution of real messages and cover traffic, the random choices of $turn$ values, and the public parameters, the real execution of the protocol and $S$'s transcripts are distributed identically. Therefore, $S$ accurately simulates the real execution of the protocol.

% Since $S$ relies only on inputs available to the ideal functionality $F$ and accurately simulates the real execution of the protocol, this show that the protocol is secure.

% % 1. Hybrid where (some) dummy messages are replaced with real messages -> this is the real execution
% % 2. simulation halts after t rounds
% % Aborts? What if A gives illegal instructions? i.e. it says that a device that does not exists should send data. S (and the real protocol) could abort. It is probably easier to have some sort of default behavior - i.e. do nothing. We can do this because nothing in our protocol relies on waiting for someone else to do something.
% % when concatenating to the transcript, A should probably be able to specify the order that things are concatenated (otherwise the distribution of the order of neighbors is probably not the same as the real execution of the protocol) - or have $S$ do it randomly?
% % S runs in polynomial time (in the number of time epochs, total number of nodes in list of graphs, and arbitrary commands of A) - do we need to say that A can't tell S to have one of the malicious nodes do an exponential amount of work?

\noindent Our goal is to show that $\forall A$ $\exists$ \ms{Sim} $\forall$ \ms{choices} such that  \ms{View_A}$(<\calA, H(choices)>)$ $\approx$ \ms{View_A}$(<\calA, Sim>)$, where $A$ is the adversary, \ms{Sim} is an efficient simulator, \ms{choices} are the states of honest parties in the protocol, $H$ is the honest parties, and $H(choices)$ are the honest parties running in the real protocol.
% I'm confused on exactly what H is

\noindent We will now construct \ms{Sim} through a series of hybrids.

\noindent \textbf{World 0}: The Real World \\
Here $A$ participates in the real protocol with real honest users.

\noindent \textbf{World 1}: Encryptions of 0 \\
\neil{S makes all of the honest parties and has their secret info} \\
Here, $A$ interacts with a simulator \ms{Sim_{0}} that simulates the behavior of honest parties by replacing all messages not to or from $A$ with encryptions of 0. In the execution of the real protocol, real messages and cover traffic (0 encrypted with a dummy key) are indistinguishable due to the properties of the underlying cipher, as long $A$ does not control the sender or receiver of the message. If $A$ controls the sender or receiver, then $A$ either knows that it sent the message or will be able to successfully decrypt the message.

\noindent \textbf{World 2}: Adding the ideal functionality \\
%H is the honest parties and they exist outside of Sim. Sim does not have access to their secret info \\
We now construct \ms{Sim}, which has the same interface to $A$ as the real protocol and has the ability to interact with the ideal functionality $F$. $H$ interacts directly with $F$ and \ms{Sim} does not have access to the secrets of parties in $H$.

\includegraphics[width=.7\linewidth]{Figures/Simulator Diagram.drawio.png}

\noindent \ms{Sim} is a white box simulator with complete knowledge of $A$. \ms{Sim} is given a list of public parameters that include $send\_rate$, $DS_{share}$, $time\_to\_keep$, and the number of time epochs $t$ to simulate. \ms{Sim} knows the list of corrupted devices $M$ with arbitrarily chosen $turn$ values, $DS$s, and public/secret key pairs for each device.

\noindent\ms{Sim} initializes the message history transcript $transcript$ to a list containing $t$ empty sets. These sets will store $(encryption, sender, receiver)$.

% registration
\noindent \ms{Sim} needs to handle the registration phase of $F$ for $A$. \ms{Sim} does this by sending a list of public keys under $A$'s control to $F$ and marking them as under $A$'s control. \ms{Sim} then receives the $turn$ values of honest parties from $F$.

\noindent\ms{Sim} does the following for each time epoch $i$ in $[1, ..., t]$:

% how to handle A adding honest vs malicious nodes?
% A sends new graph
\noindent\ms{Sim} checks the state of $G$ and saves it as $G_i$.

\noindent\ms{Sim} processes the following events as follows:

\begin{adjustwidth}{1cm}{}
% messages from $A$
\noindent (1) When a message arrives from $A$, \ms{Sim} checks $A$'s state to see what the plaintext message $message$ is and what the recipient's public key $recipient$ is. \ms{Sim} then sends $(message, recipient)$ to $F$ and records this in $transcript$.

\noindent (2) When $F$ delivers $(message, recipient)$ to \ms{Sim}, \ms{Sim} encrypts $message$ under $recipient$ and sends this to $A$. \ms{Sim} records this in $transcript$. \ms{Sim} is able to do this because $F$ delivers messages for $A$'s devices to \ms{Sim} and \ms{Sim} know's $A$'s public keys.

\noindent (3) In order to handle messages from honest parties to honest parties, \ms{Sim} is able to calculate each round which messages would be sent by honest parties based on $G_i$, messages from $A$ (forwarding), and the list of $turn$ values provided by $F$. For each of these messages, \ms{Sim} sends $A$ an encryption of 0 and records it in $transcript$.



\end{adjustwidth}

==> wrapped_figures.tex <==
\begin{figure*}
\begin{minipage}[t]{0.66\textwidth}
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.47\textwidth}
         \centering
    	 \includegraphics[width=\linewidth]{compare_DS_low.pdf}
         \caption{95th Percentile Bandwidth for various \ms{DS} exchange intervals at lower spacings. All slopes are negative, but the slope starts to flatten out at a spacing of 10 ft.}
         \label{fig:ds_low}
     \end{subfigure}
     \hfill
    \begin{subfigure}[b]{0.47\textwidth}
         \centering
    	 \includegraphics[width=\linewidth]{compare_DS_high.pdf}
         \caption{95th Percentile Bandwidth for various \ms{DS} exchange intervals at a higher spacing of 15 ft. The slope is now positive.}
         \label{fig:ds_high}
     \end{subfigure}
     \hfill
        \caption{All models ran for 5 minutes and sent messages every 30 seconds. At lower spacings, increasing the \ms{DS} exchange interval lowers the bandwidth used by devices, increasing the capacity of the system. At higher spacings, increasing the \ms{DS} exchange interval increases the bandwidth used by devices, decreasing the capacity of the system. Therefore, the optimal \ms{DS} exchange interval depends on the spacing of participants in the protest.}
        \label{fig:bitlist_effects}
\end{figure*}
\end{minipage}

\begin{minipage}[t]{0.33\textwidth}
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{delivery_compare_bitlists_minutes_5_numDevices_1600_move_False_uniform_True_broadcastType_smart_uniformSpacing_15_sendRate_30000_altlegend.pdf}
    \caption{Delivery CDF for various \ms{DS} exchange intervals. All models ran for 5 minutes, had a spacing of 15 ft., and sent messages every 30 seconds. Increasing the \ms{DS} exchange interval causes longer delivery time for messages because each message must ``wait'' longer before traversing each hop in the network. This can cause a trade-off between capacity and message delivery time for certain network configurations.}
    \label{fig:bitlist_delivery}
    % \vspace{-4em}
\end{figure}
\end{minipage}
\end{figure*}
